Business in the Grid

From 2004 to 2007 the Business In the Grid (BIG) project took place and was driven by the following goals: Firstly, make business aware of Grid technology and, secondly, try to explore new business models. We disseminated Grid computing by mainly concentrating on the central European market and interviewed several companies in order to gain insights into the Grid acceptance in industrial environments. In this article we present the results of the project, elaborate on a critical discussion on business adaptations, and describe a novel dynamic authorization workflow for business processes in the Grid.

==> abstract.tex <==
\begin{abstract}

The BIG Project was funded by the Austrian National Bank (OeNB) via
the OeNB Anniversary Fund for the following time: 1 January 2004 - 31
December 2005. The following report lists the achievement of the
project during this period.

\end{abstract}


==> survey.tex <==


Partnership with CAS - mention this and also that results have been sent to them.



